Rationalizing Neural Predictions

Prediction without justification has limited applicability. As a remedy, we learn to extract pieces of input text as justifications -- rationales -- that are tailored to be short and coherent, yet sufficient for making the same prediction. Our approach combines two modular components, generator and encoder, which are trained to operate well together. The generator specifies a distribution over text fragments as candidate rationales and these are passed through the encoder for prediction. Rationales are never given during training. Instead, the model is regularized by desiderata for rationales. We evaluate the approach on multi-aspect sentiment analysis against manually annotated test cases. Our approach outperforms attention-based baseline by a significant margin. We also successfully illustrate the method on the question retrieval task.

==> conclusion.tex <==
\section{Conclusion}
We propose a novel modular neural framework to automatically generate concise yet sufficient text fragments (i.e rationales) to justify predictions made by neural networks. The model can be trained in the end-to-end fashion, requiring no explicit annotation of rationales. We successfully illustrate the capacity of the model in two real-world applications.
